Compositional Synthesis of Leakage Resilient Programs

A promising approach to defend against side channel attacks is to build programs that are leakage resilient, in a formal sense. One such formal notion of leakage resilience is the n-threshold-probing model proposed in the seminal work by Ishai et al. In a recent work, Eldib and Wang have proposed a method for automatically synthesizing programs that are leakage resilient according to this model, for the case n=1. In this paper, we show that the n-threshold-probing model of leakage resilience enjoys a certain compositionality property that can be exploited for synthesis. We use the property to design a synthesis method that efficiently synthesizes leakage-resilient programs in a compositional manner, for the general case of n > 1. We have implemented a prototype of the synthesis algorithm, and we demonstrate its effectiveness by synthesizing leakage-resilient versions of benchmarks taken from the literature.

==> Makefile <==
# A standard Makefile for latex stuff; this can be used as a template. 

ALL = lr-lncs.pdf
GRAPHS = 
PAPERTYPE = letter

all: $(ALL)

.SUFFIXES: .pic .tex .ps .dvi .bib .bbl

%.ps: %.dvi $(GRAPHS)
	@# Using "-Ppdf" is supposed to make the PDF come out better,
	@# but it seems to screw up a few symbols in the PS file.
	@# FIX: Use -G0 as an argument to dvips!  See below.
	dvips -Ppdf -G0 -t $(PAPERTYPE) $< -o $@

%.pdf: %.ps
	ps2pdf14 -dPDFSETTINGS=/prepress -dEmbedAllFonts=true $<

#%.bbl: %.bib
#        @@echo Building bibliography...
#        BIBINPUTS=$(BIBINPUTS):./bibs bibtex $(<:.bib=)

# %.bbl: %.bib
# 	bibtex $(<:.bib=)

#%.dvi: %.tex %.bbl
lr-lncs.dvi: lr-lncs.tex macros.tex lr-lncs.bbl fig1.eps fig2.eps fig3.eps fig4.eps fig5.eps fig6.eps fig7.eps appendix.tex bench-monolithic-xc30-2to4-ie-od.tex bench-compositional-xc30-ie-od.tex
	latex $<
	@if [ "`grep 'undefined' $(<:.tex=.log)`" != "" ] ; \
	then \
	  # echo bibtex $(<:.tex=);\
	  # bibtex -min-crossrefs=99 $(<:.tex=);\
	  echo latex $<;\
	  latex $<;\
	fi
	@if [ "`grep 'undefined' $(<:.tex=.log)`" != "" ] ; \
	then \
	  # echo bibtex $(<:.tex=);\
	  # bibtex -min-crossrefs=99 $(<:.tex=);\
	  echo latex $<;\
	  latex $<;\
	fi
	@if [ "`grep 'undefined' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo latex $<;\
	  latex $<;\
	fi
	@# Anything undefined past here is really undefined
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo latex $<;\
	  latex $<;\
	fi
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo latex $<;\
	  latex $<;\
	fi
	@if [ "`grep 'may have changed' $(<:.tex=.log)`" != "" ] ; \
	then \
	  echo latex $<;\
	  latex $<;\
	fi

clean:
	-rm -f *.aux *.dvi *.log *.blg

veryclean: clean
	-rm -f *.ps *.pdf

